Neighborhood-aware Scalable Temporal Network Representation Learning

Temporal networks have been widely used to model real-world complex systems such as financial systems and e-commerce systems. In a temporal network, the joint neighborhood of a set of nodes often provides crucial structural information useful for predicting whether they may interact at a certain time. However, recent representation learning methods for temporal networks often fail to extract such information or depend on online construction of structural features, which is time-consuming. To address the issue, this work proposes Neighborhood-Aware Temporal network model (NAT). For each node in the network, NAT abandons the commonly-used one-single-vector-based representation while adopting a novel dictionary-type neighborhood representation. Such a dictionary representation records a downsampled set of the neighboring nodes as keys, and allows fast construction of structural features for a joint neighborhood of multiple nodes. We also design a dedicated data structure termed N-cache to support parallel access and update of those dictionary representations on GPUs. NAT gets evaluated over seven real-world large-scale temporal networks. NAT not only outperforms all cutting-edge baselines by averaged 1.2% and 4.2% in transductive and inductive link prediction accuracy, respectively, but also keeps scalable by achieving a speed-up of 4.1-76.7x against the baselines that adopt joint structural features and achieves a speed-up of 1.6-4.0x against the baselines that cannot adopt those features. The link to the code: https: //github.com/Graph-COM/Neighborhood-Aware-Temporal-Network.

==> 00-introduction-prev1.tex <==
\section{introduction}
 
 
Networks provide fundamental abstraction to study complex systems by viewing interacting elements as nodes and their interactions as links between nodes~\cite{newman2003structure}. Temporal networks track the interactions over time, which allows for more elaborate investigation of the dynamics of these systems~\cite{holme2012temporal,kovanen2011temporal}. How to model such dynamics to make inference over these networks has attracted much attention~\cite{snijders2010introduction,snijders2001statistical}. However, most works only focus on low-order patterns, \textit{e.g.}, link prediction between pairs of nodes~\cite{liben2007link,rahman2016link,zhu2016scalable,ma2017nonnegative,ma2018graph}. 


Many real-world systems consist of higher-order patterns that appear among more than two nodes and reflect much more complicated structures~\cite{benson2016higher,li2017inhomogeneous}: For example, in social networks, an individual can extend his/her social circles by being connected to another person, which contains only one pattern (Fig.~\ref{fig:illu} a). In contrast, when we investigate the social circle of a family with two people, it may be extended by adding one that either only one family member knows (Fig.~\ref{fig:illu} b) or both members know. The later case could be even more complicated, as it can be the case either the family members get to know the new one simultaneously (Fig.~\ref{fig:illu} d), say by inviting him/her to the family party, or via different social occasions (Fig.~\ref{fig:illu} c). To fully differentiate all the higher-order patterns, temporal links that happen in the same event should be formulated as a hyperedge (or a simplicial complex), which gives a hypergraph view of the network. Benson et al. studied the evolution of these patterns in the new view of both social and biological networks and confirmed their value of indicating domain-specific dynamics~\cite{benson2018simplicial}. %s are used to model high-order interactions that appear in a single even.   
Therefore, it is significant to build a model to predict higher-order patterns in hypergraphs, if one wants to learn the dynamics of different complex systems. A successful model may further benefit many group-targeted applications, such as group recommendation~\cite{amer2009group} or monitoring synergic actions of multiple genes~\cite{perez2009understanding}. 

%names these patterns as (b) wedge, (c) open triangle, (d) simplicial closure and

However, predicting higher-order patterns in temporal hypergraphs is challenging. To the best of our knowledge, no previous works can do so. The subtle difference among those patterns (Fig.~\ref{fig:illu} b-d) may need a model with strong representation power. Manually-design features are typically not enough. Heuristic metrics proposed for link prediction~\cite{liben2007link} have been generalized for higher-order link prediction in static networks~\cite{lahiri2007structure,benson2018simplicial,nassar2019pairwise,nassar2020neighborhood,yoon2020much}. Although the correlation between these heuristics and the higher-order patterns gets demonstrated~\cite{benson2018simplicial,yoon2020much}, the obtained performance marginally outperforms a random guessing baseline and is far from ideal to be used in practical systems.  

Neural networks due to their expressiveness have more potential to encode structural information~\cite{hamilton2017representation}. But higher-order dynamics entangles structural and temporal patterns and introduces additional challenges also for neural encoders. Recent works focused on predicting only specific higher-order patterns in either static networks~\cite{rossi2019higher,yadati2020nhp,cotta2020unsupervised,alsentzer2020subgraph}, or a few network snapshots~\cite{meng2018subgraph}.  %or single links in temporal networks~\cite{pareja2020evolvegcn,manessi2020dynamic,goyal2020dyngraph2vec,hajiramezanali2019variational,sankar2020dysat,trivedi2017know,trivedi2019dyrep,kumar2019predicting,xu2020inductive}. 
%Both  higher-order patterns with 
%Neither the full band of higher-order patterns nor elaborate temporal information get modelled properly. 
None of previous methods (either heuristic ones or neural networks) can be used to predict the entire spectrum of higher-order patterns (\textit{e.g.,} Fig.~\ref{fig:illu} b-d) let alone their evolution in the continuous time space. 

Here, we propose a novel neural network model, termed \textbf{HI}gher-order \textbf{T}emporal structure predictor (\proj) to predict higher-order network structures in continuous time space. For a proof of the concept, we focus on modeling the phenomenon of expending connection among three nodes as the patterns illustrated in Fig.~\ref{fig:illu}, also known as the procedure from an single link to a wedge, an open triangle or simplicial closure~\cite{benson2018simplicial}. The idea can be further generalized to learn more complicated patterns among more nodes. 

The key intuition of \proj is to properly encode the contextual temporal structure around three nodes of interest via neural networks and predict the future evolving patterns among them (Fig.~\ref{fig:model}). Because of the repetitive edges in temporal networks, the contextual structure could be much denser than static networks. Therefore, it is not scalable to digest the entire contextual structure and encode it via graph neural networks (GNN)~\cite{scarselli2008graph}. Instead, \proj samples and encodes a few {\em \underline{temporal random walks}} (TRW) to represent the structure. These TRWs start from those three nodes of interest and backtrack over time to collect structural and temporal features. Furthermore, to model the fundamental dynamics of each domain which is irrelevant node-personalized behaviors, \proj will remove node identities. This design guarantees good generalization of the model: The patterns extracted can be inductively applied across the network or even to other networks that share the similar dynamics. To compensate the loss of information by removing node identities, we generalize the {\em \underline{distance encoding}} technique (DE)~\cite{li2020distance} to encode each node that lies on the sampled temporal random walks. The original DE was used to improve the power of GNN to represent static networks. Our new DE is particularly designed for the temporal higher-order networks: Our DE is built upon the counts that one node appears at a certain position according to the set of sampled TRWs while leveraging a novel encoder to incorporate certain {\em asymmetry} to fit the higher-order patterns. Finally, \proj just needs to encode each DE-based TRW and then aggregate all TRWs to obtain the final representation for prediction. We conclude our contributions as the follows:

\begin{enumerate}[leftmargin=*]
    \item \proj is the first model to predict elaborated higher-order patterns in expanding connection from a single link to simplicial closure (Fig.~\ref{fig:illu} b-d). \proj achieves significant boost in predicting accuracy (xxx\%-xxx\% in AUC) compared to previous baselines that are used to predict some of these patterns.    
    \item \proj is the first model to predict higher-order network structures in continuous time space. \proj can also provide elaborate estimation of the time when different patterns in expanding connection may appear. 
    \item As \proj removes node identities and encodes TRW separately, it can automatically learn how different types of TRWs are most indicative to different higher-order patterns, which provide certain interpretation. We obtain the three data insights: 1) xxx 2) xxx 3) xxx.
\end{enumerate}







% Motivation: 
% \begin{itemize}
% \item From low-order to Higher-order study: Scope from traditional link prediction to higher-order structure prediction. Predict more complex higher-order behaviors: 1) For two people that are friends, will they get to know common friend in the future? Will they get to know the new friend in the same party or in two separate parties? When will they get to know this new friend? ... 

% \item Network dynamics methods: Improvetraditional basic statistic methods to neural methods --- Free from feature engineering: Does traditional metrics like common neighbors/A.A. scores/... still work in this much more complex cases? Can we even break these heuristics?

% \item Methodological contribution: Inspired by the distance encoding to model the correlation between more than 2 nodes. Our method can be viewed as a generalized version of the most recent casual anonymous work for pairwise nodes. 

% \item Insight contribution: Can we provide certain interpretation of our results?

% \end{itemize}

% Contributions:
% \begin{itemize}
% \item We are the first one to predict higher-order structures in dynamic graphs. Some works just considered predict higher-order structures in static graphs.

% \item Other dynamic network representation method can also be used for higher-order structure predictions. However, our neural methods are the ones that indeed capture the dynamics. Predict pairwise like -> simplicial complex closure, pairwise link prediction, wedge prediction... Predict accurate time.   

% \item Traditional scores: Common neighbors, xx, give pretty much random predictions, which kind of contradicts Benson's statement, as our problem is much more challenging. 

% \item Neural encoded features are indeed useful. Some two pieces insight from our interpretation results. We may expect our framework to help more domain scientists understand features.  
% \end{itemize}

==> 00-introduction-prev2.tex <==
%  \vspace{-4mm}

\setlength{\columnsep}{15pt}
\section{introduction}
%  \vspace{-2mm}
\pan{Why is neighborhood important? Motif features. Dynamics}
\pan{Previously neighbor info is compressed, fail. node ambiguity (TGN, TGAT, DyRep...), or over-squashing -> TGN, DyRep }
\pan{CAW, sampling, slow}
\pan{Neighbor cache, fast}
\pan{Most likely, I will rewrite the introduction but it is nice that you have done one version that helps with organizing you thoughts.}
\pan{The first paragraph explains why temporal networks are important, why processing temporal networks are hard. Temporal networks are .... They are difficult to deal with because.... So recent works consider using representation learning.}

Graphs structured data are ubiquitous and graphs that evolve are especially common in real-world settings. Social networks, citation networks, neuron activations, etc are all dynamic graphs where nodes emerge, disappear and interact with each other from time to time. Although the study on graph representation learning has been abundant and extensive since the introduction of graph neural networks (GNNs), these methods fail to capture the dynamics in graphs. In recent years, research on GNNs that leverage the temporal patterns in graphs, also called temporal GNNs (T-GNNs) \cite{nguyen2018continuous, wang2020inductive, xu2020inductive, tgn_icml_grl2020, kumar2019predicting, trivedi2019dyrep}, has become increasingly popular. These models are capable of learning a representation that combines the structural and temporal information to be used for downstream tasks, such as link predictions. \pan{Can we also deal with node classification tasks?} However, they either fail to represent important graph structures or consume too much computation or memory to be applied to large-scale datasets or real-time inference. 

\pan{The second paragraph is to introduce the issues of previous representation learning methods for temporal networks. 1. Track node representations across the time: Use NN to update one node's own features (JODIE, DyRep, TGN). Problems: Information over-squashing; Not good for inductive across the time and networks.}

\pan{Here, we need a figure to explain the over-squashing induced non-inductiveness problem. }

Similar to traditional GNNs, the core of most T-GNNs can be abstracted as message passing components \pan{We come to the terminology too fast}. Each message-passing step samples the direct neighbors of a node and then aggregates the messages of the neighbors to form a neighborhood representation. To represent a larger neighborhood with a longer diameter, these models stack multiple message-passing layers to let the information flow from the distanced neighbors to the center recursively. However, this method has been proved to be flawed.
Firstly, according to the study On the bottleneck of GNNs \cite{alon2021on}, it suffers from an information bottleneck. As aggregating messages of a node's neighbors, multiple embeddings have to be merged into one of the same dimensions. Propagating messages for multiple hops by stacking layers further squashes their representations significantly because the nodes they can reach grow nearly exponentially with the number of hops. It is described as the over-squashing effect in the study for static graphs.

\pan{Other methods do not track but adopt backtrack sampling. Problems: Avoid Information over-squashing, Good for inductive, ambiguity problems (TGAT) (similar to the node automorphism in static graphs). 3. Backtrack sampling + Motif features. Solve ambiguity problem (CAW). All backtrack sampling suffers from scalability issue, especially for online inference. Constructing motif features is even slower...}

\pan{Here, we need a figure to explain motif features and ambiguity problem.}

Furthermore, most message-passing GNNs are proved to be bounded by the 1-Weisfeiler-Lehman (WL) test for graph isomorphism such that they fail to distinguish nodes with the same graph structure without taking hints from extra features \cite{xu2019how}. So are most T-GNNS, for example, in figure 1. Suppose this is a social graph, according to the law of triadic closure or the feed-forward control, the models are likely going to predict there is a third link between A, B, and D, F. However, they are also going to predict a link between D, B and A, F because without extra information, nodes C and E, nodes A and D, and nodes B and F have the same graph structures, i.e. are isomorphic and should have the same embeddings. \underline{Implication on inductive capability?} In the study on static graphs, multiple methods are proposed to solve this issue on static graphs such as P-GNNs \cite{you2019position} and DE-GNNs \cite{li2020distance}. Commonly, they all take into account the nodes' distances or relative positions to other nodes in the graph. These additional features help the models outperform the 1-WL test. These properties are also important for dynamic graphs but most existing T-GNNs methods are not capable of capturing them.
\begin{figure}
    % \centering
    % \vspace{-5mm}
    % \includegraphics[trim={2.1cm 14.3cm 11.7cm 4.6cm},clip,width=0.5\textwidth]{TGAT-issue.pdf}
\includegraphics[width=0.3\textwidth]{tgnn-fails.png}
%   \vspace{-6.5mm}
%\hspace{-3mm}
\caption{\small{A case that fails the traditional GNNs and T-GNNs.  } }
\label{fig:t-gnn} \end{figure}
\begin{figure}
    % \centering
    % \vspace{-5mm}
    % \includegraphics[trim={2.1cm 14.3cm 11.7cm 4.6cm},clip,width=0.5\textwidth]{TGAT-issue.pdf}
\includegraphics[width=0.45\textwidth]{neighborhood cache.png}
%   \vspace{-6.5mm}
%\hspace{-3mm}
\caption{\small{The neighborhood cache that mitigates the information bottleneck.  } }
\label{fig:n-cache} \end{figure}
\begin{figure*}
    % \centering
    % \vspace{-5mm}
    % \includegraphics[trim={2.1cm 14.3cm 11.7cm 4.6cm},clip,width=0.5\textwidth]{TGAT-issue.pdf}
\includegraphics[width=1\textwidth]{MAT-arch.png}
%   \vspace{-6.5mm}
%\hspace{-3mm}
\caption{\small{\proj overall architecture.} \pan{Motif feature extraction is not very clear.} \pan{Augmented,input, hidden states are not clear.} }
\label{fig:arch} \end{figure*}



The Causal Anonymous Walk (CAW) \cite{wang2020inductive} attempts to address the graph isomorphic issue by calculating the relative node identity but it is notably slow and memory-intensive. It summarizes the relative distances from a node w to the source node u and from $w$ to the target node $v$ so that nodes $u$ and $v$ are distinguishable even they have the same local neighborhood structures. However, to achieve this, CAW has to keep track of all events for all nodes. For every training example, it backtracks the history of the nodes to sample a fixed number of neighbors and, neighbors of neighbors if multiple hops are involved. A lot of CAW's blocking operations are performed on the CPU which slows down the model overall.


\pan{Here, we propose Motif-Aware Temporal network models (\proj). The key idea is to use not only a vector representation for each node but also a set representation that track a subset of its neighbors. A set representation before pooling can naturally avoid over-squashing and can be used to construct motif features. The set representation is updated online instead of sampled for each training/testing examples. We design a dedicated pipeline to support the parallel update of the set representation. First, the set representation is sub-neighborhood and with small overhead. CAW demonstrates that subsampled motif features are sufficient to provide good performance. Second, we implement a GPU hash for efficient update. Third, to aggregate the set representation with motif features into the final prediction, we also propose a sparse attention network. }

\pan{We need a figure to introduce the model diagram.}

Therefore, although the existing SOTA models successfully incorporated temporal patterns in addition to the graph structures, they have to trade-off between learning expressivity and efficiency. To address these limitations, we propose \proj, an efficient learning framework that's more powerful than the state-of-the-art representation learning of dynamic graphs. This model comprises several key components that tackle the above challenges, the neighborhood caches, motif features constructor, and the sparse-GAT output layer \pan{What is sparse GAT layer?}. The neighborhood caches design achieves the following three purposes. 1) It serves as an up-to-date store for temporal node states. For each node, it feeds information in the latest interaction into an RNN to update the node states. 2) It alleviates the information bottleneck by expanding the number of embeddings in proportion to the number of neighbors. They increase the complexity they are capable of representing. 3) It improves efficiency by summarizing the neighborhood. It avoids backtracking history and calculating the neighborhood features in the forward propagation path of the model.



To sum up, this work 1) introduces a powerful yet efficient temporal graph neural network that can be used for inductive learning on large dynamic graphs, 2) empirically studies different components in the proposed method, and 3) concludes that it outperforms SOTA methods in either performance or efficiency or both.



==> 03-methodology_draft0.tex <==
%\vspace{-2mm}
\section{Methodology}\label{sec:method}





%\vspace{-1mm}
In this section, we introduce the framework of \proj. \pan{The crucial thing for this section is from top to bottom. First introduce the big several blocks before going into the details. Introduce why in the algorithmic level \proj is good. And then why in the }
On high-level \proj consists of three major components: the neighborhood cache, the motif features constructor, and the graph attention network. The neighborhood cache stores encoded history between node pairs. For each incoming event $(u, v, e, t)$, \proj reads the representations associated with $u$ and $v$ from the neighborhood cache. It then extracts the motif features according to the history of their surroundings and aggregates the motif-aware messages with a graph attention network to output the final predictions. Lastly, it updates the neighborhood cache for $u$ and $v$ based on this latest event.

These modules are very effective for the model performance. However, due to the extra memory and computation complexity, the model has to be fully optimized for real-world applications, including shrinking the memory consumption, simplifying computations, and parallelizing. We will study specific examples such as the GPU hashing algorithm which maximizes parallelism of a mini-batch with well-contained GPU memory and efficient GPU operations that work with sparse tensors.

%  We also provide a generic framework that is flexible to balance efficiency and performance as preferred for the downstream applications. Finally, it is extendable for further improvements for both efficiency and performance. For example, dynamic allocations of the neighborhood buffer for memory efficiency and the cache eviction algorithms to smartly discard old neighbors in favor of the new neighbors for higher quality neighborhood representation. 



\subsection{Neighborhood cache} \pan{at least 1 page}
The neighborhood cache is a fixed-size memory module in the GPU that is aimed to resolve the over-squashing issue. It is optimized for quick access and update to ensure model efficiency. We will first discuss our motivations. Then, we will explain the high level concepts of the neighborhood cache and dive deep into the efficiency considerations.


\subsubsection{Toward more expressive neighborhood representations}

Motivated by over-squashing. Why Message passing are insufficient. Why TGNs are insufficient. It motivated us to design the neighborhood cache. 

Motivated by CAWs, it can also used for extracting the motif features.

First, it keeps track of the identities of nodes' neighbors. They can be used for constructing the temporal network motifs~\cite{paranjape2017motifs}. CAW~\cite{wang2020inductive}'s outstanding performance on temporal link predictions empirically testifies that temporal motifs features are very effective. See section \ref{sec:motif} for more details regarding temporal network motifs in \proj.

Second, it stores the intermediate representations of a node and its neighborhood \pan{Not clear about this}. This idea stems from the memory module in TGN and the embedding trajectories in JODIE. Keeping neighborhood embeddings can effectively improve model efficiency so that they are faster than general message passing T-GNNs such as CAW~\cite{wang2020inductive} and TGAT~\cite{xu2020inductive}. The major computation bottleneck with message passing is they usually have to \begin {enumerate*}
\item look through the events associated with a node in the history (from latest to earliest), \item sample temporal edges, and \item aggregate the neighborhood states on the fly. \pan{The explanation clear is too much on efficiency but not enough for modeling needs.}
\end {enumerate*}

Third, we adopt a set of vectors for representing a node's local neighborhood. We reserve multiple representations for each node such that there is a vector dedicated to encoding the history between an origin node and another node in its neighborhood. There are two implications with this design. (1), it relieves the information bottleneck and avoids the over-squashing phenomenon. It is well-studied in \cite{alon2021on} that general GNNs suffer from over-squashing because all interactions within a node's neighborhood are compressed into a fixed-size vector. This issue is discovered recently and there is no solution for it yet. It might be natural to think that increasing the hidden size can reduce over-squashing but \cite{alon2021on} empirically showed that dimensionality increase is ineffective in preventing over-squashing. Instead, it shows that by adding a fully-adjacent layer in which every pair of nodes is connected by an edge, it achieves 42\% improvement \pan{improvement on what?} without adding weights. However, it is unrealistic and computationally expensive to assume that all node pairs are connected. Our vectors are more compact representations that replace this layer. (2), it allows information flow beyond direct neighbors without history backtracking, sampling, or stacking message passing layers. Although TGN avoids these steps with the memory module, it is unaware of messages beyond direct neighbors. To get information from the second-hop neighbors, it inevitably needs to do the backtracking and sampling. Therefore, we observe a massive slowdown in the two-layer TGN. Our neighborhood cache can represent messages from not only direct neighbors but also sub-neighborhood beyond the first hop.

\subsubsection{The neighborhood cache design}

neighborhood cache high level concept
neighborhood state definitions
neighborhood state update of when a new link comes in.
Not storing all edges or timestamp so use RNNs to get a summary.

It keeps track of the encoded states of a node and its neighborhood up to the current timestamp. A distinctive characteristic of this neighborhood cache that sets it apart from the memory modules in the existing methods like TGN \cite{tgn_icml_grl2020} is that it maintains a set of vectors for its neighborhood states instead of just a single compressed representation. The neighborhood cache is designed with three aspects.

\textbf{neighbor states}
% Each vector in the set of the neighborhood cache can be seen as a neighbor state which is dedicated to representing the interactions between a source node and each of its neighbors. Note that the interactions can be indirect in the case of multiple-hop neighbors.
For node $u \in \mathcal{V}$, suppose at the current time, it has formed a neighborhood with a set of nodes $\mathcal{N}(u) \subset \mathcal{V}$. Neighborhood cache for $u$ keeps track of a subset of $u$'s temporal neighbors, \textit{i.e.} $\mathcal{S}(u) \subset \mathcal{N}(u)$ and the timestamps of their interactions $\mathcal{T}(u)$. We also keep a collection of vectors and assign one vector for each of the neighbors we are keeping in $\mathcal{S}(u)$, \textit{i.e.} $\mathcal{C}(u) = \{c_{u,v} | v \in \mathcal{S}(u)\}$. Each vector represents a neighbor state. We encode the history between $u$ and $v$ including the link features and the temporal features into the neighbor state $c_{u,v}$ with RNNs. 
\begin{align}\label{eq:rnn}
    c_{u,v} = \text{RNN}(\{e_i \oplus F(t_i)\}_{i=0}^m) \text{ where } e_i \in \mathbb{R}^d
\end{align}
For $F(t)$, we leverage the random Fourier temporal features (Eq.\eqref{eq:randomf})to encode time. Since each neighbor state encodes a relationship between a node and its neighbor, a combination of neighbor states can represent the surroundings of a node more expressively.
% $c_{u,v} = e_{u,v} \oplus m_{u,v} \text{ where } \{e_{u,v}, m_{u,v}\} \in \mathbb{R}^d$. We encode the edge features along the previous interactions between $u$ and $v$ into $e_{u,v}$, while $m_{u,v}$ aggregates the temporal information extracted from the timestamps of those interactions. Altogether, $c_{u,v}$ represents the state of the history . 
% for the shortest paths between the source node to other nodes as shown in Fig.\ref{fig:n-cache}.To get the representation of nodes and edges in the local neighborhood without squashing,  To control the size of the neighborhood we want to consider, we limit the shortest paths to have lengths less than $k$, where $k$ is a hyper-parameter deciding within how many hops from a node we explore.
%For $f_2(t)$, we adopt random Fourier features to encode time~\citep{xu2019self,kazemi2019time2vec} which may approach any positive definite kernels according to the Bochner’s theorem~\citep{bochner1992theorem}. 

\textbf{second-hop neighbors}
Similar to the first-hop neighbors, second hop neighbors are updated when a new event $(u,v, e, t)$ comes in. We can directly sample the first-hop neighbors of $v$ to update the second hop states of $u$. The only caveat of this module is that the update is not real-time. $u$ is not aware of $v$'s new neighbors after they interacted until their next interaction. However, in practice, this asynchronous update can already provide meaningful performance gain. \yuhong{provide number x\%}


\pan{Efficient neighborhood cache update}
These expanded neighborhood states show potential in improving not only efficiency but also model expressivity. However, there are two fundamental challenges regarding their scalability. First, allocating one vector for each pair of nodes that interacted in the past consumes considerable memory. It is even more burdensome if the model needs to store extra representations for the second-hop neighbors. It does not scale for large networks with limited memory. 
%For example, the wiki-talk temporal dataset has more than 7 million static edges.
Second, throughout the learning process, we need to access and update this chunk of memory for all nodes in a mini-batch. It can easily become the computation bottleneck. To address these challenges, we introduce the GPU hashing algorithm for quick neighborhood cache operations. \pan{I do not think the explanation on how a node comes in and update the neighbors. So the motivation of GPU hashing is missing and unclear.}

fix size
Sampling
hashing
update in a batch
We first expose a hyperparameter $s$ to control the maximum number of unique neighbors allowed to be stored for each node such that the size of the cache can be maintained. Keeping a subset of total neighbors is similar to the sampling for GNNs' message passing. It is also sufficient for temporal motif feature construction \pan{This sentense you should introduce later when define what is motif features}. When CAW~\cite{wang2020inductive} extract network motifs, it samples temporal random walks and still achieves high performance. Our subsets of neighbors are precomputed asynchronously \pan{What do you mean by this?}, while other models need to sample edges from the history or the adjacency matrices during the learning. Even though there are some limitations which we will discuss in section \ref{sec:limit}, the neighborhood cache can work as an efficient replacement for other sampling methods. \pan{I do not think motif features are well defined.}

Now that the memory complexity of the cache is limited, we need to optimize the data structure to reduce the time complexity. It is natural to think of an origin node as the key and the set of neighbors as the value. In general, a hash map is the most efficient data structure for storing key-value pairs like these because accessing or updating a value to any key guarantees O(1) time complexity. Given that the adjacency matrices of most graphs are sparse, the variable-length sets are also suitable for storing node neighbors. However, this complex data structure does not easily fit into the GPU and thus is not optimized for parallelism.



\textbf{GPU Hashing}. We decided to design the data structure within GPU to allow parallel operations for all nodes in a mini-batch. Specifically, we allocate $|\mathcal{V}| \cdot s$ vectors in the GPU and initialize them with zeros. We store the neighbor states of a node $u$ into these vectors consecutively, so the $\{u \times s + j\}^s_{j=0}$ vectors belong to $u$'s neighborhood.
\textbf{Access}. 
To get the neighbor states associated with a node, we simply do an index read in the tensors. Since it does not guarantee that all preallocated slots are filled up with neighbors, we filter out empty vectors to reduce unnecessary computations with them. This will require downstream of the pipelines to work with unaligned tensors and we discuss some implementations for sparse tensors further in section \ref{sec:sparse}.
 \textbf{Update}
Suppose a new event with $u$ and $v$ arrives at time $t$ and we try to update the cache of $u$. We will first apply a hash function $0 <= f(v) \mod s$ to decide which position we store the representation of $c_{u,v}$ at. If the slot selected is empty or is already taken by $v$, we will simply update it with the hidden state of RNN of eq.~\ref{eq:rnn}. Otherwise, there is a hash collision with a previous link of $u$. Whether $v$ can occupy this slot is decided by a Bernoulli random variable with probability $p$.  Since more recent links are generally more informative, as shown in previous papers such as \cite{wang2020inductive}, we favor new links over old links. Thus, $p$ is a function that involves the time difference between the old link and the current link. It is proportional to $exp(\alpha, t_i - t)$ where $\alpha$ is a hyperparameter, such that older links are more likely to be evicted. These if-else conditions can be implemented by flipping the bits of a boolean tensor. When there are multiple events associated with the same node, it will store only one update nondeterministically. See alg \ref{alg:update}
Both the access and the update operations are all done within the GPU so can be parallelized for a mini-batch of events.
\begin{algorithm}
        \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
        $\textbf{h} \leftarrow hash(\textbf{v}) \mod s$ \;
        $\textbf{h} \leftarrow \textbf{h} + s \cdot \textbf{u} $\;
        $\textbf{o} \leftarrow \:\textcircled{$\neg$}\:((\mathcal{S}(\textbf{u})[\textbf{h}] \:\textcircled{$=$}\: \vec{\textbf{0}}) \:\textcircled{$\lor$}\: (\mathcal{S}(\textbf{u})[\textbf{h}] \:\textcircled{$=$}\: \textbf{v}))$\;
        $\textbf{r} \leftarrow [(d_i \sim U[0,1]) > exp(\alpha, T(\textbf{u})[i] - t)]_{i=0}^\text{batch size}$\;
        $\textbf{r} \leftarrow \:\textcircled{$\neg$}\:(\textbf{o} \:\textcircled{$\wedge$}\: \textbf{r}) $\;
        $\mathcal{S}(\textbf{u})[\textbf{h}] \leftarrow \textbf{v} \odot \textbf{r}$\;
        $\mathcal{C}(\textbf{u})[\textbf{h}] \leftarrow \textbf{c}$\;
        $\mathcal{T}(\textbf{u})[\textbf{h}] \leftarrow t$\;
        \caption{\small{Neighborhood Cache Batch Update ($\textbf{u}$, $\textbf{v}$, $t$, $\mathcal{C}(\textbf{u})$, $\mathcal{S}(\textbf{u})$, $\mathcal{T}(\textbf{u})$, $\alpha$, $\textbf{c}$)
        \newline Note: $hash$, \textcircled{$\neg$}, \textcircled{$=$}, \textcircled{$\wedge$}, \textcircled{$\lor$}, $\odot$ are pointwise operations }}\label{alg:update}
        \end{algorithm}
        



\subsection{Relative temporal motifs}\label{sec:motif} \pan{at least 0.5 page}

\subsubsection{The effective temporal motif features}
CAW shows that motif features are effective for distinguishing isomorphic nodes.
However, sampling is especially slow, so we leverage the neigbhorhood cache.

cross join
how to explain this?
\subsubsection{Relative motif extraction}
relative node identity.
anonymization.


\subsection{sparse implementation}\label{sec:sparse}  \pan{ One paragraph}

get from neighborhood cache

relative temporal aggregation

GAT layer with scattered

\subsubsection{sparse message passing}
\subsubsection{sparse GATs}
\subsubsection{sparse neighborhood store updates}


\subsection{Complexity analysis}

\subsection{limitations and discussions}\label{sec:limit}
3 hops. variable length neighbor. more strategic eviction.
\subsection{\yuhong{Questions}}
what should we aggregate what should not?

The motifs I can get are not exactly temporal network motifs because they are not aware of the ordering of the links. Does it matter?

Can 2nd hop hidden state of a node use the 1st hop hidden states of its direct neighbors?
Test \proj with initializing 2nd hop with default?


OGN mentions TGN also need to keep the history and sample edges. need to verify.

 There are other heuristics we can explore such as taking the number of interactions in the past in to account.

==> 03-methodology_draft1.tex <==
\section{Methodology}\label{sec:method}

In this section, we introduce the framework of \proj.
In the high level \proj consists of three major components: the neighborhood cache, the motif features constructor, and the graph attention network. The neighborhood cache stores encoded history between node pairs. For each incoming event $(u, v, e, t)$, \proj reads the representations associated with $u$ and $v$ from the neighborhood cache. It then extracts the motif features according to the history of their surroundings and aggregates the motif-aware messages with a graph attention network to output the final predictions. Lastly, it updates the neighborhood cache for $u$ and $v$ based on this latest event.

These modules are very effective for the model performance. However, due to the extra memory and computation complexity, the model has to be fully optimized for real-world applications, including shrinking the memory consumption, simplifying computations, and parallelizing for a mini-batch. We will study specific examples such as the GPU hashing and GPU inner join algorithms  which maximize parallelism of a mini-batch with well-contained GPU memory. \pan{Good}

\subsection{Neighborhood cache}\label{sec:neighborhood}
The neighborhood cache is a fixed-size memory module in the GPU that aims to resolve the over-squashing issue \pan{and structural feature construction }. It is optimized for quick access and update to ensure model efficiency. We will first discuss motivations. Then, we will explain the high level concepts of the neighborhood cache and dive deep into the efficiency considerations.


\subsubsection{Toward more expressive neighborhood representations}
The neighborhood cache is primarily motivated by the over-squashing effect of message passing. \pan{Okay, here MP does not need to review again?} Message passing (MP) is widely used for both static and dynamic graph learning~\cite{kipf2016semi, velivckovic2018graph, xu2020inductive}. It is a neural network architecture that allow messages of nodes in a graph to flow to neighboring nodes. Each node starts with a hidden representation $h$ and an MP layer aggregates hidden states of neighboring nodes to update its own representation. Each MP layer lets information flows one step in the network. By stacking multiple layers, it makes the node representation incorporate more information coming from neighbors of longer distances. While it has advantage in being aware of the structural information around the node, it introduces an information bottleneck described as the over-squashing phenomenon~\cite{alon2021on}.
\textbf{over-squashing} is well-studied in \cite{alon2021on} that general GNNs suffer from over-squashing. Since $k$-layer MP propagates information from all nodes in a $k$-hop neighborhood into a target node and squashes it into one fix-sized vector, it is going to lose some information inevitably. Over-squashing is more obvious if $k$ is larger because the number of representations it has to compress into a single vector grows exponentially with the neighborhood distance. From another perspective, representations of distanced neighbors have to go through multiple squashing before reaching the target node and the their information will be harder to generalize. As a result, over-squashing prevents GNNs from fitting the training data well, especially for nodes with rich connections.

Inspired by this novel explanation for GNNs under-fitting, we explore a way to relieve the information bottleneck \pan{Try to use another term} by avoiding squashing as much as possible. It is already shown in~\cite{alon2021on} that increasing the dimension of the destination vector is not an effective solution \pan{Interesting things}. Thus, we first increase the representation power for node neighborhood by increasing the number of vectors. Instead of representing a node, the vectors represent relationships or links between nodes. We term each vector as a \textit{relation state}. Without any quashing, a relation state can represent a part of a neighborhood on its own. A complete set of relation states associated with a node can represent the relationship between the node and its entire neighborhood. In the context of temporal network, each relation state summarizes the historical interactions between a pair of nodes.  

Formally, suppose at the current time $t$, node $u \in \mathcal{V}$, has formed a neighborhood with a set of nodes $\mathcal{N}(u) \subset \mathcal{V}$. A collection of relation states around $u$ can be represented as $\mathcal{C}(u) = \{c_{(u,v)} | v \in \mathcal{N}(u)\}$. Initialize as $c^{(0)}$ In order for $c_{(u,v)}$ to represent the relationship between $u$ and $v$, we need to leverage both the edge features and the temporal information in the history. We propose using RNNs to encode the interactions overtime. RNNs have the inductive bias of forgetting long-term memory in favor of the more recent one . It is well-suited for encoding temporal information in graphs because more recent links are generally more informative as shown in previous papers such as \cite{wang2020inductive}. We define
\begin{align}\label{eq:rnn}
    c_{u,v} = \text{RNN}(\{e_i \oplus F(t_i)\}_{i=0}^m) \text{ where } e_i \in \mathbb{R}^d
\end{align}
For $F(t)$, we leverage the random Fourier temporal features (Eq.\eqref{eq:randomf}) to encode time.
The relation states associated with a node can be used as features and fed into any pooling layer to get the final representation of the node.


\subsubsection{The introduction of neighborhood cache}
 A straight forward implementation of a model that incorporates the relation states would be as follow:\pan{I do not think it is necessary to say so much on naive implementation.}
 When the representation of a node $u$ at time $t$ is requested,
 \begin{enumerate}
     \item Sampling: sample a set of $u$'s neighbors from the adjacency matrix.
     \item Backtracking: for each $v \in \mathcal{N}_u$, look up the historical links between $u$ and $v$ to find out all interactions before $t$
     \item Encoding: for each $v \in \mathcal{N}_u$, encode the history between $u$ and $v$ with RNNs
 \end{enumerate}
 The problem with this method is that we need to repeat these steps for every training example, even for nodes we have calculated before. They become significant computation bottleneck. Thus we propose neighborhood cache for storing the intermediate results to avoid repetitive computations. It is an optimized module within the GPU that achieves O(1) parallel access and update for a mini-batch.
 
We first expose a hyperparameter $s$ to control the maximum number of unique neighbors allowed to be stored for each node such that the size of the cache can be maintained. We then allocate $s \times |\mathcal{V}|$ vectors in the GPU and initialize with zeros. We reserve $s$ vectors for each node $u \in \mathcal{V}$ for storing the relation states with neighboring nodes of $u$. The relation states for each node are stored consecutively, so the $\{u \times s + j\}^s_{j=0}$ vectors belong to $u$'s neighborhood. We denote the collection of these vectors as $\mathcal{C}$. To identify the opposite \pan{opposite?} node of the relation states, we also store a list of neighbor identities $\mathcal{S}$ in the same order as $\mathcal{C}$. The neighbor identities are also going to be used for calculating the relative temporal motifs (Sec. \ref{sec:motif}).

 \textbf{Update and eviction} We train the model with events in the order of time so that we can update the relation states as time progresses. Suppose a new event with $u$ and $v$ arrives at time $t$ and we try to update the cache of $u$. We will first apply a hash function $0 <= f(v) < s$ to decide which position we store the representation of $c_{u,v}$ at. If the slot selected is empty or is already taken by $v$, we will simply update it with the hidden state of RNNs of eq.~\ref{eq:rnn}. Otherwise, there is a hash collision with a previous neighbor $n_i \in \mathcal{N}_u$ of $u$. Whether $v$ can occupy this slot is decided by a Bernoulli random variable with probability $p$. $p$ is a function that involves the time difference between the old link and the current link. To promote new links and evict old ones, $p$ is proportional to $exp(\alpha, t_i - t)$ where $\alpha$ is a hyperparameter and $t_i$ is the timestamp of the interaction with the existing neighbor $n_i$. We store the latest timestamps of the interaction with neighbors $\mathcal{S}$ in another set $\mathcal{T}$. These if-else conditions can be implemented by flipping the bits of a Boolean tensor. When there are multiple events associated with the same node, it will store only one update nondeterministically (Alg \ref{alg:update}).

\begin{algorithm}
        \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
        $\textbf{h} \leftarrow hash(\textbf{v}) \mod s$ \;
        $\textbf{h} \leftarrow \textbf{h} + s \cdot \textbf{u} $\;
        $\textbf{o} \leftarrow \:\textcircled{$\neg$}\:[[\mathcal{S}[\textbf{h}] \:\textcircled{$=$}\: \vec{\textbf{0}}] \:\textcircled{$\lor$}\: [\mathcal{S}[\textbf{h}] \:\textcircled{$=$}\: \textbf{v}]]$\;
        $\textbf{r} \leftarrow [(d_i \sim U[0,1]) > exp(\alpha, \mathcal{T}[\textbf{h}_i] - t)]_{i=0}^\text{batch size}$\;
        $\textbf{r} \leftarrow \:\textcircled{$\neg$}\:(\textbf{o} \:\textcircled{$\wedge$}\: \textbf{r}) $\;
        $\mathcal{S}[\textbf{h}] \leftarrow \textbf{v} \odot \textbf{r}$\;
        $\mathcal{C}[\textbf{h}] \leftarrow \textbf{c}$\;
        $\mathcal{T}[\textbf{h}] \leftarrow t$\;
        \caption{\small{Neighborhood Cache Batch Update ($\textbf{u}$, $\textbf{v}$, $t$, $\mathcal{C}$, $\mathcal{S}$, $\mathcal{T}$, $\alpha$, $\textbf{c}$)
        \newline Note: $hash$, \textcircled{$\neg$}, \textcircled{$=$}, \textcircled{$\wedge$}, \textcircled{$\lor$}, $\odot$ are pointwise operations \pan{These signs are not widely used.}}}\label{alg:update}
        \end{algorithm}
    
\textbf{Access}. 
Through the training of a batch, we need to access the neighborhood cache once to get all relation states associated with a node. We simply do an index read in the tensors. Since it does not guarantee that all preallocated slots are filled up with neighbors, we filter out empty vectors to reduce unnecessary computations. Given that the number of neighbors for each node is different, it will require downstream of the pipelines to work with unaligned vectors. We discuss an efficient algorithm that smoothly operates these vectors in section \ref{sec:motif}.\pan{Here saying to postpone the intro in 4.2 is not good.}

\textbf{Beyond direct neighbors}
To avoid sampling, we also allocate a fixed-number set of vectors for each node to represent longer distance neighbors. Intuitively, this is similar to \cite{gilmer2017neural}'s virtual edges for shortening long distances and avoiding over-squashing. We use second-hop neighbors for illustration.  Similar to direct neighbors, second-hop neighbors are also updated when a new event $(u, v, e, t)$ comes in. We can directly sample the first-hop neighbors of $v$ to update the second hop states of $u$. The only caveat of this module is that the update is not real-time. $u$ is not aware of $v$'s new neighbors after they interacted until their next interaction. In practice, this asynchronous update can already provide significant performance gain. \yuhong{provide number x\%}. It also naturally captures the causality which we will explore in Sec.\ref{sec:motif}. Finally, this method can also be extended to any $k$-hop neighbors.
 



\subsection{Relative temporal motifs}\label{sec:motif} \pan{at least 0.5 page}
In order to distinguish nodes with similar local structures, we integrate the relative temporal motifs encoding between the source and the target nodes of an event into the link prediction model. This can be seen as an analogy to the distance encoding in the static GNNs~\cite{li2020distance}.
To extract the motif features, we leverage temporal walks. This is an idea inspired by CAW~\cite{wang2020inductive}. However CAW is inefficient because it samples random walks for each node by backtracking over time to extract motifs. To avoid backtracking, we leverage the neighborhood cache (Sec. \ref{sec:neighborhood}).

\subsubsection{Encoding of a powerful structural feature}
We are interested in temporal motifs because they capture both the structural patterns and the temporal information. To abstract temporal motif features, we start with temporal walks. Although temporal walks resemblance the temporal motifs, temporal walks have explicit node identities and timestamps such that they do not generalize as well as temporal motifs. An important step toward transforming temporal walks to temporal motifs is anonymization of nodes and abstraction of timestamps.

We cannot simply remove node identities from temporal walks because a walk contains structural information that is related to node identities. We propose anonymizing node identities with distance encoding (DE) \cite{li2020distance}. There are different DE variants. We will focus on the shortest path distance (SPD) because it is the simplest while it does not perform worse than other methods in practice.
The SPD of node $a$ in a set of temporal walks $S=\{W_1, W_2, ..., W_M\}$ is defined as
\begin{equation}
    \tilde{g}(a; S)\triangleq i,
    \text{where } i=\min\{j|\exists W\in S, a \text{ appears at }W[j]\}. 
    \label{eq:spd}
\end{equation} 
To abstract timestamps, we only need to keep track of the order in which the edges
occur as described in \cite{paranjape2017motifs}. Because temporal walks follow edges in the descending order of time, they naturally encode the temporal structure. Thus, we can simply drop the timestamps of temporal walks.


\subsubsection{extracting motifs from neighborhood cache}
While the most straight forward approach to obtain the temporal walks is the temporal random walk proposed in~\cite{wang2020inductive}, it requires backtracking history and sampling walks which lead to computation bottleneck. Thus, we leverage the neighborhood cache to avoid random walk sampling. Because we update and evict neighbors with randomness, and keep direct and $2^{nd}$ hop neighbors in separate caches, they naturally represent a fragmented random walk. Furthermore, thanks to our delayed update of multiple-hop neighbors, the links to the 2-nd hop neighbors usually appear earlier and therefore, they follow the temporal ordering of temporal walks. Since neighborhood cache is aware of the distances of the neighbors to the source node, we can easily arrive at the SPD of nodes in temporal walks.

\begin{figure}
\includegraphics[width=0.45\textwidth]{Relative motifs.png}
%   \vspace{-6.5mm}
%\hspace{-3mm}
\caption{\small{Left: the neighbors stored in the caches. Assume it is storing the complete neighbors. Middle: the subgraphs inferred from a single source, either A or B. Right: the sub-graphs inferred combining neighborhoods of both A and B. Note that anonymizing the node ids in the subgraphs produces the motifs. } }
\label{fig:relative} \end{figure}

We have been talking about generating motif features from a single source node. However, it is not sufficient as shown in (Fig.\ref{fig:relative}. Given neighbor ids $\textbf{s}_u$, we can infer an incomplete subgraph around $u$. However, it can miss important structural information because (1), the neighborhood is incomplete. we sample the neighbors and our update beyond first hop is delayed. (2), The neighborhood cache is not aware of the links between the neighbors.
Thus, if the opposite node $v$ happens to be one of the neighbors of $u$, we can fill in missing links and expand the neighborhood. The motifs extracted from this augmented subgraph -- termed relative motifs, are far more informative than motifs of a single source. As an example, Fig.\ref{fig:relative} demonstrates that single-source subgraphs do not capture the the link (B,C) and (C,D) while the combined subgraph does. We will empirically compare the motif features with single source v.s. the relative motifs features. CAW has also showed that the random walks from a single source is insufficient while merges random walks from both sources boosts the model performance.


Alg.~\ref{alg:motif} introduces the algorithm to extract relative motif feature from the sub-neighborhoods of source node $u$ and target $v$, i.e. $\textbf{s}_u$ and $\textbf{s}_v$ retrieved from the neighborhood cache. The vector operations can all be done within the GPU and thus can be parallelized for a mini-batch. All $\textbf{g}^{(i,j)}_u$ can be used as features to calculate $u$'s final embedding.
\begin{algorithm}
\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
 \For{$i$ from $1$ to $m$, the $i-$th step}{
    $l \leftarrow \textit{one hot}(i)$\;
    $\textbf{l}^{(i)}_u \leftarrow
  \bigl[ \underbrace{%
    l \quad  l \quad  \cdots \quad  l
  }_{\text{$|\textbf{s}^{(i)}_u| $~elements}} \bigr]$\;
  $\textbf{l}^{(i)}_v \leftarrow
  \bigl[ \underbrace{%
    l \quad  l \quad  \cdots \quad  l
  }_{\text{$|\textbf{s}^{(i)}_v| $~elements}} \bigr]$\;
 }
 
 \For{$i$ from $1$ to $m$, the $i-$th step}{
    \For{$j$ from $1$ to $m$, the $j-$th step}{
        $\textbf{s}_{all} \leftarrow [\textbf{s}^{(i)}_u ||  \textbf{s}^{(j)}_v]$\;
        $\textbf{uni}, \textbf{idx} \leftarrow $ find unique elements in $\textbf{s}_{all}$; also return original indices of the unique elements\;
        $\textbf{l}_{all} \leftarrow [\textbf{l}^{(i)}_u || \textbf{l}^{(j)}_v]$\;
        $\textbf{f}^{(i,j)} \leftarrow \bigl[ \underbrace{%
    0 \quad  0 \quad  \cdots \quad  0
  }_{\text{$|\textbf{uni}| $~elements}} \bigr]$\;
        Scatter add $\textbf{l}_{all} $ to $\textbf{f}^{(i,j)}$ according to indices in $\textbf{idx}$\;
        $\textbf{g}^{(i,j)} \leftarrow \bigl[ \underbrace{%
    0 \quad  0 \quad  \cdots \quad  0
  }_{\text{$|\textbf{idx}| $~elements}} \bigr]$\;
        Assign elements in $\textbf{f}^{(i,j)} $ to $\textbf{g}^{(i,j)}$ according to indices in $\textbf{idx}$\;
        $\textbf{g}^{(i,j)}_u \leftarrow \textbf{g}^{(i,j)}[1, 2, \quad \cdots \quad , |\textbf{s}^{(i)}_u|]$\;
        $\textbf{g}^{(i,j)}_v \leftarrow \textbf{g}^{(i,j)}[|\textbf{s}^{(i)}_u|, |\textbf{s}^{(i)}_u| + 1, \quad \cdots \quad, |\textbf{s}^{(j)}_v|]$\;
    }
 }
\caption{\small{Relative motifs aggregation ($\textbf{s}_u$, $\textbf{s}_v$, $m$) }}\label{alg:motif}
\end{algorithm}

\subsection{Graph attention output layer}
We propose a simple single-layer GAT~\cite{velivckovic2018graph} to summarize the neighbors information conveyed by the relation states and the relative motif features and generate a final node representation. We layout all neighbors sampled and treat them all as the direct neighbors. Following GAT, we will first calculate the attention scores with 
\begin{align}\label{eq:attention}
    \alpha_{ij} = \frac{exp(\text{LeakyReLU}(\textbf{a}^T[\textbf{W}\textbf{h}_i||\textbf{W}\textbf{h}_j]))}
    {\sum_{k\in \mathcal{N}_i} exp(\text{LeakyReLU}(\textbf{a}^T[\textbf{W}\textbf{h}_i||\textbf{W}\textbf{h}_k]))}
\end{align}
where \textbf{a} is a learnable weight vector of a single-layer feedforward neural network, \textbf{W} is a weight matrix that project input features into higher-level features, one for each attention head.

Next, we aggregate the projected features according to the attention score and produce the final embedding. Formally, it can be expressed as:
\begin{align}\label{eq:final_sum}
    \textbf{o}_i = \sigma(\sum_{j\in \mathcal{N}_i}\alpha_{ij} \textbf{W}\textbf{h}_j)
\end{align}
where $\sigma$ is a nonlinearity activation.

Here we also leverage the scatter add method so we can parallelize all nodes in a mini-batch even though the number of neighbors are unaligned for the nodes.
